Controllability of the 1D Schr\"odinger equation using flatness

We derive in a direct way the exact controllability of the 1D free Schr\"odinger equation with Dirichlet boundary control. We use the so-called flatness approach, which consists in parametrizing the solution and the control by the derivatives of a "flat output". This provides an explicit and very regular control achieving the exact controllability in the energy space.

==> Computation.tex <==

\section{Computation Fourier}
A Faire:
\begin{itemize}
\item fourier convergence, OK
\item formula for phase 1 solution  and its derivatives (recurrence) in terms of special function (for asymptotics)
\item computation of phase 2: recurrence for gevrey step, recurrence for flat output, derivatives of product
\end{itemize}




the integral $\theta^-(t,1)$ is difficult to evaluate numerically when $t$ is small (the integrand oscillates very fast)


An idea is to expand the initial condition as a Fourier sine series, namely
\begin{IEEEeqnarray}{rCl}\label{eq:Fourier}
	\theta_0(x) &=& \sum_{n\ge1}c_n\sqrt2\sin(n\pi x),
\end{IEEEeqnarray}
and use the truncated control $T_{\bar n}(t,1)$ defined by
\begin{IEEEeqnarray*}{rCl}
	T_{\bar n}(t,x) &:=& \sum_{1\le n\le\bar n}c_n\theta^-_n(t,x)\\
	%
	\theta^-_n(t,x) &:=& \int_{-1}^1E(t,x-y)\sin(n\pi y)dy.
\end{IEEEeqnarray*}
Indeed $\theta^-_n$ can be expressed with special functions (to do)

We must prove it makes sense
As $\theta_0\in L^2(0,1)$, the equality \eqref{eq:Fourier} holds in the $L^2$ sense,
\begin{IEEEeqnarray*}{rCl}
	\lim_{\bar n\to\infty}\norm{\theta_0-S_{\bar n}}_{L^2(0,1)} &=& 0,
\end{IEEEeqnarray*}
where $S_{\bar n}(x):=\sum_{1\le n\le\bar n}c_n\sqrt2\sin(n\pi x)$, and $\sum_{n\ge1}\abs{c_n}^2=\norm{\theta_0}^2<\infty$.

\begin{prop}\mbox{}
\begin{enumerate}[(i)]
\item\label{it:C} $\lim_{\bar n\to\infty}T_{\bar n}=\theta^-$ in $\mathcal{C}\bigl(\Rset;L^2(0,1)\bigr)$
%
\item\label{it:H} $\lim_{\bar n\to\infty}T_{\bar n}=\theta^-$ in $\mathcal{C}\bigl(\Rset\setminus(-\tau,\tau);H^r(0,1)\bigr)$
for all $\tau>0$ and $r\in\Nset$
\end{enumerate}
\end{prop}
%
\begin{pf}

 

\begin{IEEEeqnarray*}{rCl}
	\IEEEeqnarraymulticol{3}{l}{\norm{\theta^-(t,\cdot)-T_{\bar n}(t,\cdot)}_{L^2(0,1)}}\\ \quad
	&=& \biggnorm{\int_{-1}^1E(t,\cdot-y)\bigl(\theta_0(y)-S_{\bar n}(y)\bigr)^{odd}dy}_{L^2(0,1)}\\
	%
	&\le& \biggnorm{\int_{-1}^1E(t,\cdot-y,t)\bigl(\theta_0(y)-S_{\bar n}(y)\bigr)^{odd}dy}_{L^2(\Rset)}\\
	%
	&=& 2\norm{\theta_0-S_{\bar n}}_{L^2(0,1)}
\end{IEEEeqnarray*}
where we have used~\ref{}. This means $\theta^-(t,\cdot)$ tends to $S_{\bar n}(t,\cdot)$ in $L^2(0,1)$, uniformly in~$t$, which is~\eqref{it:C}.

\begin{IEEEeqnarray*}{rCl}
	\IEEEeqnarraymulticol{3}{l}{\norm{\partial_x^k\bigl(\theta^-(t,\cdot)-T_{\bar n}(t,\cdot)\bigr)}_{L^2(0,1)}}\\ \quad
	&=& \biggnorm{\int_{-1}^1\partial_x^kE(t,\cdot-y)\bigl(\theta_0(y)-S_{\bar n}(y)\bigr)^{odd}dy}_{L^2(0,1)}\\
	%
	&\le& K_k\biggnorm{\int_{-1}^1E(t,\cdot-y)\bigl(\theta_0(y)-S_{\bar n}(y)\bigr)^{odd}dy}_{L^2(\Rset)}\\
	%
	&\le& 2K_k\norm{\theta_0-S_{\bar n}}_{L^2(0,1)},
\end{IEEEeqnarray*}
with $K_k:=(4\tau)^{-\frac{k}{2}}\sup_{\abs z\leq\frac{1}{\sqrt\tau}}\abs{H_k(z)}$; we have used \eqref{eq:derE} then~\ref{}. This means $\partial_x^k\theta^-(t,\cdot)$ tends to $\partial_x^kS_{\bar n}(t,\cdot)$ in $L^2(0,1)$, uniformly in~$t$, which obviously implies~\eqref{it:C}.
%
\qed\end{pf}

We can now estimate the error between the true solution and the approximate solution $\hat{\theta^-}$
\begin{cor} The error with truncated control is 
\begin{IEEEeqnarray*}{rCl}
	\norm{\theta^-(\tau,\cdot)-T_{\bar n}(\tau,\cdot)}_{L^\infty(0,1)}
	&\le& M\sum_{n>\bar n}\frac{\abs{c_n}}{n}
\end{IEEEeqnarray*}
\begin{IEEEeqnarray*}{rCl}
	\norm{\theta^-(\tau,\cdot)-\widehat{\theta^-}(\tau,\cdot)}_{L^\infty(0,1)}
	&\le& M\sum_{n>\bar n}\frac{\abs{c_n}}{n}
\end{IEEEeqnarray*}
utile?
\begin{IEEEeqnarray*}{rCl}
	\norm{\partial_x^k\bigl(\theta^-(\tau,\cdot)-T_{\bar n}(\tau,\cdot)\bigr)}_{L^\infty(0,1)}
	&\le& M_k\sum_{n>\bar n}\frac{\abs{c_n}}{n}
\end{IEEEeqnarray*}

\end{cor}

\begin{pf}

Tn is the solution

the series Tn
normal convergence, hence its limit $T_\infty(t,\cdot)$ is continuous and by previous prop is $\theta^-(t,\cdot)$
%$T_\infty(t,x)=\theta^-(t,x)$

CAUTION: exchange integral and sum possible if H1 (somme des coeff converge absolument)
\begin{IEEEeqnarray*}{rCl}
	\norm{\theta^-(\tau,\cdot)-T_{\bar n}(\tau,\cdot)}_{L^\infty(0,1)}
	&=& \Bignorm{\sum_{n>\bar n}c_n\theta_n^-(\tau,\cdot)}_{L^\infty(0,1)}
\end{IEEEeqnarray*}

since $\theta_n^-(\tau,\cdot)\sim\frac{K}{n}$ for $n$ large (integration by parts)
%
\qed\end{pf}


==> Estimates.tex <==
\section{Estimates}

\begin{itemize}
\item ideal trajectory $\theta$ and ideal control $u$, defined in theorem~\ref{thm:Main}
%
\item truncated trajectory $\theta_{\bar n,\bar j}$ and truncated control $u_{\bar n,\bar j}$ defined by
\begin{IEEEeqnarray*}{rCl}
	Y_{\bar n}(t) &:=& \phi_s\Bigl(\frac{t-\tau}{T-\tau}\Bigr)\partial_xT_{\bar n}(t,0)\\
	%
	\theta_{\bar n,\bar j}(t,x) &:=& 
	\begin{dcases*}
	\theta_{\bar n}(t,x) & if $0\le t\le\tau$,\\
	\sum_{j\le\bar j}\frac{(-i)^jx^{2j+1}}{(2j+1)!}Y_{\bar n}^{(j)}(t) & if $\tau<t\le T$
	\end{dcases*}\\
	%
	u_{\bar n,\bar j}(t) &:=& \theta_{\bar n}(t,1)
\end{IEEEeqnarray*}
%
\item actual trajectory $\tilde\theta_{\bar n,\bar\jmath}$ obtained by applying the truncated control $u_{\bar n,\bar j}$
\end{itemize}

REM: truncated control regular at $t=\tau$??? Si, comme dans preuve du theoreme

$t\ge\tau$ dans la suite

\begin{IEEEeqnarray*}{rCl}
	\norm{\theta(t,\cdot)-\theta_{\bar n,\bar j}(t,\cdot)}_{L^\infty(0,1)}
	&\le& bornes\\
	%
	\norm{\theta-\theta_{\bar n,\bar j}}_{W^{q,\infty}(\tau,T)\times(0,1)}
	&\le& bornes\\
	%
	\norm{u-u_{\bar n,\bar j}}_{W^{q,\infty}(0,1)}
	&\le& bornes
\end{IEEEeqnarray*}


\begin{IEEEeqnarray*}{rCl}
	I_{n\pm}(t,x) 
	&:=& \int_{-1}^1E(t,x-y)e^{\pm in\pi y}dy
\end{IEEEeqnarray*}


\begin{IEEEeqnarray*}{rCl}
	\partial_x^kI_{n\pm}(t,x) &=& \int_{-1}^1\partial_x^kE(t,x-y)e^{\pm in\pi y}dy\\
	%
	&=& (-1)^k\int_{-1}^1\partial_y^kE(t,x-y)\frac{d}{dy}\biggl(\frac{e^{\pm in\pi y}}{\pm in\pi}\biggr)dy\\
	%
	&=& \frac{(4it)^{-\frac{k}{2}}}{\pm in\pi}\left[H_k\biggl((x-y)\sqrt{\frac{i}{4t}}\biggr)E(t,x-y)e^{\pm in\pi y}\right]_{-1}^1
	\\&&\quad+\>\frac{1}{\pm in\pi}\partial_x^{k+1}I_{n\pm}(t,x)
\end{IEEEeqnarray*}
where we have integrated by parts and used~\eqref{eq:derE}.

\begin{IEEEeqnarray*}{rCl}
	\partial_x^{2l}I_{n\pm}(t,0) &=& 0+\frac{1}{\pm in\pi}\partial_x^{k+1}I_{n\pm}(t,0)\\
	%
	\partial_x^{2l+1}I_{n\pm}(t,0) &=& 2(-1)^n\frac{(4it)^{-\frac{2l+1}{2}}}{\mp in\pi}H_{2l+1}\biggl(\sqrt{\frac{i}{4t}}\biggr)E(t,1)
	\\&&\quad+\>\frac{1}{\pm in\pi}\partial_x^{2l+2}I_{n\pm}(t,0)
\end{IEEEeqnarray*}
since $H_{2l}$ is even, $H_{2l+1}$ is odd, and $E$ is even w.r.t its second argument


since $\partial_t\theta^-_n=i\partial^2_x\theta^-_n$,



